Formal Support for Standardizing Protocols with State

Many cryptographic protocols are designed to achieve their goals using only messages passed over an open network. Numerous tools, based on well-understood foundations, exist for the design and analysis of protocols that rely purely on message passing. However, these tools encounter difficulties when faced with protocols that rely on non-local, mutable state to coordinate several local sessions. We adapt one of these tools, {\cpsa}, to provide automated support for reasoning about state. We use Ryan's Envelope Protocol as an example to demonstrate how the message-passing reasoning can be integrated with state reasoning to yield interesting and powerful results. Keywords: protocol analysis tools, stateful protocols, TPM, PKCS#11.

==> msg_based.tex <==
\section{A Purely Message-Based Analysis}
\label{msg_based}

The transition relation for the simplified TPM implicitly defines the
set of paths---that is, sequences of states---that are allowed by the
TPM's interface. In particular, a path for this TPM model is any
sequence of hash chains, each starting from the known boot value
$\cn{d}_0$. This set of paths constrains what the other protocol
participants can see and do when interacting with the device. 

An analysis of the Envelope Protocol requires an execution semantics
that accounts for 
\begin{enumerate}
\item the exact set of paths allowed by our model of the TPM,
\item the ways in which these possible paths constrain behavior when
  they synchronize with the transmission of protocol messages, and
\item the adversary's inability to access the state directly.
\end{enumerate}
%
Given our representation of state as messages, it is natural to wonder
if we might be able to achieve these properties in a purely
message-based semantics. If so, that would mean that many tools that
already exist could be applied directly to the analysis of stateful
protocols without modification. Unsurprisingly, however, it turns
out that a message-based semantics is insufficient, but understanding
how it falls short is instructive for identifying relevant axioms for
stateful analyses. We thus use the rest of this section to describe an
attempt to analyze the Envelope Protocol using only the transmission
and reception of messages. 

The fundamental observation for trying to model state in a
message-based semantics is that long-term state could be viewed as a
communication channel between local sessions that have access to the
state. Reading the state corresponds to receiving a message on this
channel, and writing or updating the state corresponds to sending a
message on this channel. We might therefore represent the transition
relation using pairs of events; $m_0\trans m_1$ would be represented
by the reception of message $m_0$ followed by the transmission of
message $m_1$. This would help satisfy Condition~1 above. 

However, since the adversary is assumed to have access to message
channels, we must modify this approach in order to satisfy
Condition~3. We may posit that encrypting the state messages with a
key that is unknown to the adversary can satisfy Condition~3 since the
adversary will never be able to access the plaintext. We might also
worry that these state messages could be delivered to non-state
reception events thereby not respecting Condition~2. This can be
prevented by ensuring the encrypted states all contain a tag constant
$\tg{0}$ that identifies them as states and they all use a key that
can be syntactically distinguished from keys used for other purposes,
e.g. by hashing.

The result for a transition $m_0\trans m_1$ would be
%
$$-\enc{\tg{0},m_0}{\#k}\Rightarrow+\enc{\tg{0},m_1}{\#k}$$
%
where the $-/+$ notation denotes message reception and transmission
respectively, and $\Rightarrow$ denotes (local) succession of events.
\begin{figure*}[t]
\ifart
\[
\begin{array}{l}
  \fn{boot}(k\typ\srt{S}, p\typ\top)={}\\
  \quad\inbnd\cn{g}_3\Rightarrow\inbnd
  \enc{\tg{0}, p}{\#k}\Rightarrow\outbnd\enc{\tg{0},
    \cn{s}_0}{\#k}\\[1.2ex]

  \fn{extend}(\mathit{sid}\typ\srt{D}, \mathit{tpmk}\typ\srt{A},
  \mathit{esk},k\typ\srt{S},p,t\typ\top)={}\\
  \quad\inbnd (\cn{g}_4,\mathit{tpmk},
  \enc{\mathit{esk}}{\mathit{tpmk}}) \Rightarrow
  \outbnd (\cn{g}_4, \mathit{sid}) \Rightarrow
  \inbnd\enc{\cn{g}_5,t,\mathit{sid}}{\mathit{esk}}\\
  \qquad\Rightarrow\inbnd
  \enc{\tg{0},p}{\#k} \Rightarrow\outbnd\enc{\tg{0},
    \#(t,p)}{\#k}\\[1.2ex]

  \fn{quote}(k\typ\srt{S}, \mathit{aik}\typ\srt{A},
  p,n\typ\top)={}\\
  \quad\inbnd  (\cn{g}_6,n)\Rightarrow\inbnd\enc{\tg{0},p}{\#k}\Rightarrow
  \outbnd\enc{\tg{0},p}{\#k}\Rightarrow \outbnd
  \enc{\cn{g}_6,p,n}{\mathit{aik}}\\[1.2ex]

  \fn{decrypt}(m,t\typ\top, k',\mathit{aik}\typ\srt{A}, k\typ\srt{S})={}\\
  \quad\inbnd (\cn{g}_7,\enc{m}{k'})\Rightarrow\inbnd
  \enc{\cn{g}_8, k', p}{\mathit{aik}}\Rightarrow \inbnd
  \enc{\tg{0},p}{\#k}\Rightarrow \outbnd \enc{\tg{0},p}{\#k}
  \Rightarrow \outbnd m\\[1.2ex]

  \fn{createkey}(k,\mathit{aik}\typ\srt{A}, t\typ\top)={}\\
  \quad\inbnd
  (\cn{g}_9, t)\Rightarrow \outbnd \enc{\cn{g}_8, k,
    t}{\mathit{aik}}
\end{array}
\]
\begin{center}
  \fbox{
    \begin{tabular}{llllllllll}
      $\cn{g}_0$&state&
      $\cn{g}_2$&refuse&
      $\cn{g}_4$&session&
      $\cn{g}_6$&quote&
      $\cn{g}_8$&created\\
      $\cn{g}_1$&obtain&
      $\cn{g}_3$&boot&
      $\cn{g}_5$&extend&
      $\cn{g}_7$&decrypt&
      $\cn{g}_9$&create key
    \end{tabular}
  }
\end{center}
\else
\begin{center}
\begin{minipage}{0.7\textwidth}
$$
\begin{array}{l}
  \fn{boot}(k\typ\srt{S}, p\typ\top)={}\\
  \quad\inbnd\cn{g}_3\Rightarrow\inbnd
  \enc{\tg{0}, p}{\#k}\Rightarrow\outbnd\enc{\tg{0},
    \cn{s}_0}{\#k}\\[1.2ex]

  \fn{extend}(\mathit{sid}\typ\srt{D}, \mathit{tpmk}\typ\srt{A},
  \mathit{esk},k\typ\srt{S},p,t\typ\top)={}\\
  \quad\inbnd (\cn{g}_4,\mathit{tpmk},
  \enc{\mathit{esk}}{\mathit{tpmk}}) \Rightarrow
  \outbnd (\cn{g}_4, \mathit{sid}) \Rightarrow
  \inbnd\enc{\cn{g}_5,t,\mathit{sid}}{\mathit{esk}}\\
  \qquad\Rightarrow\inbnd
  \enc{\tg{0},p}{\#k} \Rightarrow\outbnd\enc{\tg{0},
    \#(t,p)}{\#k}\\[1.2ex]

  \fn{quote}(k\typ\srt{S}, \mathit{aik}\typ\srt{A},
  p,n\typ\top)={}\\
  \quad\inbnd  (\cn{g}_6,n)\Rightarrow\inbnd\enc{\tg{0},p}{\#k}\Rightarrow
  \outbnd\enc{\tg{0},p}{\#k}\Rightarrow \outbnd
  \enc{\cn{g}_6,p,n}{\mathit{aik}}\\[1.2ex]

  \fn{decrypt}(m,t\typ\top, k',\mathit{aik}\typ\srt{A}, k\typ\srt{S})={}\\
  \quad\inbnd (\cn{g}_7,\enc{m}{k'})\Rightarrow\inbnd
  \enc{\cn{g}_8, k', p}{\mathit{aik}}\Rightarrow \\
  \qquad\inbnd
  \enc{\tg{0},p}{\#k}\Rightarrow \outbnd \enc{\tg{0},p}{\#k}
  \Rightarrow \outbnd m\\[1.2ex]

  \fn{createkey}(k,\mathit{aik}\typ\srt{A}, t\typ\top)={}\\
  \quad\inbnd
  (\cn{g}_9, t)\Rightarrow \outbnd \enc{\cn{g}_8, k,
    t}{\mathit{aik}}
\end{array}
$$
\end{minipage}\quad
\begin{minipage}{0.20\textwidth}
  \fbox{\begin{tabular}{ll}
    $\cn{g}_0$&state\\
    $\cn{g}_1$&obtain\\
    $\cn{g}_2$&refuse\\
    $\cn{g}_3$&boot\\
    $\cn{g}_4$&session\\
    $\cn{g}_5$&extend\\
    $\cn{g}_6$&quote\\
    $\cn{g}_7$&decrypt\\
    $\cn{g}_8$&created\\
    $\cn{g}_9$&create key
  \end{tabular}
}
\end{minipage}
\end{center}
\fi
\caption{State-Bearing Traces}\label{fig:state roles}
\end{figure*}

\begin{figure*}[t]
\ifart
\[
\begin{array}{l}
  \fn{boot}(k\typ\srt{S}, p\typ\top)={}\\
  \quad\inbnd\cn{g}_3\Rightarrow\inbnd
  \enc{\tg{0}, p}{\#k}\Rightarrow\outbnd\enc{\tg{0},
    \cn{s}_0}{\#k}\\[1.2ex]

  \fn{extend}(\mathit{sid}\typ\srt{D}, \mathit{tpmk}\typ\srt{A},
  \mathit{esk},k\typ\srt{S},p,t\typ\top)={}\\
  \quad\inbnd (\cn{g}_4,\mathit{tpmk},
  \enc{\mathit{esk}}{\mathit{tpmk}}) \Rightarrow
  \outbnd (\cn{g}_4, \mathit{sid}) \Rightarrow
  \inbnd\enc{\cn{g}_5,t,\mathit{sid}}{\mathit{esk}}\\
  \qquad\Rightarrow\inbnd
  \enc{\tg{0},p}{\#k} \Rightarrow\outbnd\enc{\tg{0},
    \#(t,p)}{\#k}\\[1.2ex]

  \fn{quote}(k\typ\srt{S}, \mathit{aik}\typ\srt{A},
  p,n\typ\top)={}\\
  \quad\inbnd  (\cn{g}_6,n)\Rightarrow\inbnd\enc{\tg{0},p}{\#k}\Rightarrow
  \outbnd\enc{\tg{0},p}{\#k}\Rightarrow \outbnd
  \enc{\cn{g}_6,p,n}{\mathit{aik}}\\[1.2ex]

  \fn{decrypt}(m,t\typ\top, k',\mathit{aik}\typ\srt{A}, k\typ\srt{S})={}\\
  \quad\inbnd (\cn{g}_7,\enc{m}{k'})\Rightarrow\inbnd
  \enc{\cn{g}_8, k', p}{\mathit{aik}}\Rightarrow \inbnd
  \enc{\tg{0},p}{\#k}\Rightarrow \outbnd \enc{\tg{0},p}{\#k}
  \Rightarrow \outbnd m\\[1.2ex]

  \fn{createkey}(k,\mathit{aik}\typ\srt{A}, t\typ\top)={}\\
  \quad\inbnd
  (\cn{g}_9, t)\Rightarrow \outbnd \enc{\cn{g}_8, k,
    t}{\mathit{aik}}
\end{array}
\]
\begin{center}
  \fbox{
    \begin{tabular}{llllllllll}
      $\cn{g}_0$&state&
      $\cn{g}_2$&refuse&
      $\cn{g}_4$&session&
      $\cn{g}_6$&quote&
      $\cn{g}_8$&created\\
      $\cn{g}_1$&obtain&
      $\cn{g}_3$&boot&
      $\cn{g}_5$&extend&
      $\cn{g}_7$&decrypt&
      $\cn{g}_9$&create key
    \end{tabular}
  }
\end{center}
\else
\begin{center}
\begin{minipage}{0.7\textwidth}
$$
\begin{array}{l}
  \fn{boot}=\stinit\cn{g}_0\\[1.2ex]

  \fn{extend}(\mathit{sid}\typ\srt{D}, \mathit{tpmk}\typ\srt{A},
  \mathit{esk}\typ\srt{S},p,t\typ\top)={}\\
  \quad\inbnd (\cn{g}_4,\mathit{tpmk},
  \enc{\mathit{esk}}{\mathit{tpmk}}) \Rightarrow
  \outbnd (\cn{g}_4, \mathit{sid}) \Rightarrow
  \inbnd\enc{\cn{g}_5,t,\mathit{sid}}{\mathit{esk}}\\
  \qquad\Rightarrow\tran(p,\#(t,p))\\[1.2ex]

  \fn{quote}(\mathit{aik}\typ\srt{A},
  p,n\typ\top)=\inbnd(\cn{g}_6,n)\Rightarrow
  \obsv p\Rightarrow \outbnd\enc{\cn{g}_6,p,n}{\mathit{aik}}\\[1.2ex]

  \fn{decrypt}(m,t\typ\top, k,\mathit{aik}\typ\srt{A})={}\\
  \quad\inbnd (\cn{g}_7,\enc{m}{k})\Rightarrow\inbnd
  \enc{\cn{g}_8, k, p}{\mathit{aik}}\Rightarrow
  \obsv p\Rightarrow \outbnd m\\[1.2ex]

  \fn{createkey}(k,\mathit{aik}\typ\srt{A}, t\typ\top)=
  \inbnd(\cn{g}_9, t)\Rightarrow \outbnd \enc{\cn{g}_8, k,
    t}{\mathit{aik}}
\end{array}
$$
\end{minipage}\quad
\begin{minipage}{0.20\textwidth}
  \fbox{\begin{tabular}{ll}
    $\cn{g}_1$&origin\\
    $\cn{g}_1$&obtain\\
    $\cn{g}_2$&refuse\\
    $\cn{g}_3$&boot\\
    $\cn{g}_4$&session\\
    $\cn{g}_5$&extend\\
    $\cn{g}_6$&quote\\
    $\cn{g}_7$&decrypt\\
    $\cn{g}_8$&created\\
    $\cn{g}_9$&create key
  \end{tabular}
}
\end{minipage}
\end{center}
\fi
\caption{Stateful Traces}\label{fig:stateful roles}
\end{figure*}

Using these receive-transmit pairs of state-bearing messages the TPM
roles are represented in Fig.~\ref{fig:state roles}, where tag
$\cn{g}_1$ is obtain and tag $\cn{g}_2$ is refuse.  In the \fn{extend}
role, we now show the two initial messages that provide replay
prevention; the TPM supplies a fresh nonce as a session ID that must
appear with the value to be extended into the PCR.  The \fn{createkey}
role does not interact with the state. It simply creates a key that
will be constrained by the state in the boot role.

%\ifllncs\enlargethispage{2ex}\fi
Alice's role, including the messages to prevent replays, is:
$$
\begin{array}{l}
  \fn{alice}(\mathit{sid},v\typ\srt{D},\mathit{esk}\typ\srt{S},
  k,\mathit{tpmk},\mathit{aik}\typ\srt{A},n\typ\srt{E}
  \ifpriorities, p\typ\top\fi)={}\\
  \quad\outbnd (\cn{g}_4,\mathit{tpmk},
  \enc{\mathit{esk}}{\mathit{tpmk}}) \Rightarrow
  \inbnd (\cn{g}_4, \mathit{sid})\\
  \qquad \Rightarrow \outbnd
  \enc{\cn{g}_5,n,\mathit{sid}}{\mathit{esk}}
  \Rightarrow
  \outbnd(\cn{g}_9, \#(\cn{g}_1,\#(n,\initstate)))\\
  \qquad \Rightarrow
  \inbnd \enc{\cn{g}_8,\#(\cn{g}_1,\#(n,\initstate))}{\mathit{aik}}
  \Rightarrow \outbnd \enc{v}{k}
\end{array}
$$
The parameters $\mathit{sid}$ and~$\mathit{tpmk}$ help prevent
replays.  To make formulas more comprehensible, we omit them.


This section discusses how we use our analysis tool {\cpsa} to infer
results in the theory $\tbnd(\Pi)$. {\cpsa} carries out enrich-by-need
analysis, and characterizes the set of bundles consistent with a
partial description of a bundle.

These partial descriptions are called \emph{skeletons}. {\cpsa} takes
as input an initial skeleton $\skel_0$, and when it terminates it
outputs a set of more descriptive skeletons $\{\skelB_i\}_{i\in I}$.
They have the property that any bundle containing the structure in the
initial skeleton $\skel_0$ also contains all the structure in one of
the output skeletons $\skelB_i$.  In particular, it infers all of the
non-adversarial behavior that must be present in any bundle satisfying
the initial description. Of course for some initial skeletons
$\skel_0$, there may be no bundles that are consistent with them. In
this case, {\cpsa} outputs the empty set.

The security goal for the Envelope Protocol is that a run of Alice's
role should ensure that the secret and the refusal certificate are not
both available:
%
\begin{goal}\label{goal:alice}
  Consider the following events:
  \begin{itemize}
    \item An instance of the Alice role runs to completion, with
    secret $v$ and nonce $n$ both freshly chosen;
    \item $v$ is observed unencrypted;
    \item the refusal certificate \ifieeetrans
      $$\enc{\cn{\mathtt{``quote"}},
      \#(\cn{\mathtt{``refuse"}},\#(n,\fn{val})),
      \enc{v}{k'}}{\fn{aik}}$$
      \else
      $\enc{\cn{\mathtt{``quote"}},
      \#(\cn{\mathtt{``refuse"}},\#(n,\fn{val})),
      \enc{v}{k'}}{\fn{aik}}$
      \fi
      is {\ifllncs ob-\break served\else observed\fi} unencrypted.
  \end{itemize}
%
  These events, which we call jointly $\skel_0$, are not all present
  in any execution.
\end{goal}
%
We can feed {\cpsa} an input skeleton $\skel_0$ representing this
undesirable situation.
\ifllncs
\else
The skeleton~$\skel_0$ is visualized in Fig.~\ref{fig:alice pov}.
\fi

We would hope {\cpsa} could determine that no bundles are consistent
with this input $\skel_0$ and return the empty set. However, our
technique of using state-bearing messages to represent the TPM state
transitions underconstrains the set of possible state paths.  For this
reason, {\cpsa} actually produces one skeleton in its output.  This
skeleton represents some activity that must have occured within the
TPM in any bundle conforming to the initial skeleton. It contains an
instance of the decrypt role (to explain the secret leaking), an
instance of the quote role (to explain the creation of the refusal
token), and several instances of the extend role (to explain how the
TPM state evolved in order to allow the other two operations).

%Fig.~\ref{fig:state split} 
The figure (!!!\emph{which is absent because Paul didn't know how to
  port all the metapost over}!!!) displays the relevant portion of
{\cpsa}'s output displaying only the state-bearing nodes of the extend
strands inferred by {\cpsa}. Notice that two of the extend strands
branch off from the third strand. This is a state split in which a
single state evolves in two distinct ways. The technique of using
state-bearing messages is not sufficient to preclude this possibility.

% \begin{figure*}[t]
%   \begin{center}
%     \includegraphics{envelope\grphext-0.mps}
%     \caption{State Splitting}\label{fig:state split}
%   \end{center}
% \end{figure*}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "root"
%%% End:

